Beyond Human-Only: Evaluating Human-Machine Collaboration for Collecting High-Quality Translation Data

Collecting high-quality translations is crucial for the development and evaluation of machine translation systems. However, traditional human-only approaches are costly and slow. This study presents a comprehensive investigation of 11 approaches for acquiring translation data, including human-only, machineonly, and hybrid approaches. Our findings demonstrate that human-machine collaboration can match or even exceed the quality of human-only translations, while being more cost-efficient. Error analysis reveals the complementary strengths between human and machine contributions, highlighting the effectiveness of collaborative methods. Cost analysis further demonstrates the economic benefits of human-machine collaboration methods, with some approaches achieving top-tier quality at around 60% of the cost of traditional methods. We release a publicly available dataset containing nearly 18,000 segments of varying translation quality with corresponding human ratings to facilitate future research.

==> 03a_sec2a_bias_analysis.tex <==
\input{figures/fig_mt_bias_ende_metricX}

While our findings demonstrate the efficacy of human-machine collaboration in translation, it is crucial to carefully evaluate potential biases when incorporating machine-generated text, especially for evaluation datasets. This consideration is particularly important when assessing the quality of machine translation systems using metrics that may be influenced by the source of the reference translations.
 
Metric self-bias occurs when a metric favors translation text generated by the same source used for its reference translation. This phenomenon is particularly relevant when considering machine-generated data as a reference. We define metric self-bias as the discrepancy in metric scores obtained when using machine-generated versus human-generated references.

To investigate this, we demonstrate the English-German experiment in Figure ~\ref{fig:mt_bias_ende_metricx} comparing five machine translation (MT) systems: ONLINE-A, ONLINE-W, GPT-4 5shot (\textsc{BestWMT}), ONLINE-G (\textsc{MidWMT}), and Gemini-1.0 Ultra 0shot (LLMRefine). We used a high-quality human reference (\textsc{HumanRef+HumanPEx2}), strongly correlated with MQM scores (see Figure~\ref{fig:mqm-human-ref-corr}), as the unbiased baseline. This allowed us to examine the self-bias introduced when the same MT system was used for initial translation, post-editing, or both. Our analysis employed MetricX, with corresponding COMET22 results and ZhEn results are available in the Appendix.

Figure~\ref{fig:ende_bias_init_translation_metricx} highlights that MetricX assigns a significantly lower score (indicating higher quality) to GPT-4 5shot when using \textsc{BestWMT+HumanPE} as the reference compared to \textsc{HumanRef+HumanPEx2}. The bias even flips its ranking in comparison with Gemini. This similar trend is also observed for ONLINE-G.

Similarly, Figure~\ref{fig:ende_bias_post_edit_metricx} explores potential self-bias stemming from machine post-editing. However, MetricX does not assign a significantly lower score to the Gemini translation when using \textsc{HumanRef+LLMRefine} as the reference.

Figure~\ref{fig:ende_bias_combined_metricx} examines the combined impact of self-bias from both initial translation and post-editing. While a significant score difference exists for the initial translation, it is negligible for post-editors. Larger score differences indicate a stronger bias against translations generated by the same source as the reference. Thus, self-bias appears primarily driven by the initial translation, with post-editing holds minimal bias and still contributing to quality improvements.

==> figures/fig_post_edit_agree_category_ende.tex <==
\begin{figure}[htb!]
  \includegraphics[width=0.95\columnwidth]{figures/ende-post-edit-agree-category.pdf}
  \caption{Error category distribution of different agreement sections. Average percentage is reported across the three initial translation sources}
  \label{fig:ende_post_edit_agree_category}
\end{figure}




==> tables/table_ende_mqm_domains.tex <==
\begin{table}[!htb]
    \centering
    \begin{adjustbox}{width=0.98\columnwidth}
    \begin{tabular}{lccc}
        \toprule
        \textbf{Reference} & \textbf{Mastodon} & \textbf{User Review} & \textbf{News}\\
        \midrule
        \textsc{HumanRef} & 1.83 & 4.94 & 5.31 \\
        \textsc{HumanRef+HumanPE} & 1.96 & 4.39  & 4.51 \\
        \textsc{HumanRef+HumanPEx2} & 1.69 & 4.54 & 5.25 \\
        \textsc{HumanRef+LLMRefine} & 1.66 & 3.10 & 3.53\\
        \textsc{BestWMT} & 1.91 & 4.44 & 3.54 \\
        \textsc{BestWMT+HumanPE} & 1.74 & 3.08 & 4.66 \\
        \textsc{BestWMT+LLMRefine} & 2.02 & 3.67 & 4.25\\
        \textsc{MidWMT} & 3.81 & 10.89 & 6.77 \\
        \textsc{MidWMT+HumanPE} & 1.87 & 6.41 & 4.53 \\
        \textsc{MidWMT+LLMRefine} & 1.94 & 6.60 & 4.25 \\
        \textsc{OrigHumanRef} & 1.83 & 3.22 & 3.60 \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{English-German MQM human evaluations for generalMT2023 with different systems under different domains.}
    \label{tab:zhen_mqm_domains}
\end{table}

==> tables/table_ende_mtme.tex <==
\begin{table*}[!htp]
\centering
\footnotesize
\begin{tabularx}{0.75\textwidth}{lr|rrrr}
\toprule
\multicolumn{1}{l}{\bf Metric} & \multicolumn{1}{c}{\bf avg-corr} & \multicolumn{1}{c}{\bf en-de} & \multicolumn{1}{c}{\bf en-de} & \multicolumn{1}{c}{\bf en-de} & \multicolumn{1}{c}{\bf en-de}\\
\multicolumn{1}{l}{\bf level} & & \multicolumn{1}{c}{\bf sys} & \multicolumn{1}{c}{\bf sys} & \multicolumn{1}{c}{\bf seg} & \multicolumn{1}{c}{\bf seg} \\
\multicolumn{1}{l}{\bf corr{\_}fn} & & \multicolumn{1}{c}{\bf accuracy} & \multicolumn{1}{c}{\bf pearson} & \multicolumn{1}{c}{\bf pearson} & \multicolumn{1}{c}{\bf acc-t} \\
\multicolumn{1}{l}{\bf task} & & \multicolumn{1}{c}{\bf task1} & \multicolumn{1}{c}{\bf task2} & \multicolumn{1}{c}{\bf task3} & \multicolumn{1}{c}{\bf task4}\\
\midrule
\verb|MetricX_HumanRef_LLMRefine| & 0.838 & 0.985 & 0.958 & 0.569 & 0.604 \\
\verb|MetricX_HumanRef_HuamnPEx2| & 0.838 & 0.985 & 0.957 & 0.571 & 0.605 \\
\verb|MetricX_HumanRef_HumanPE|  & 0.838 & 0.985 & 0.957 & 0.57 & 0.604  \\
\verb|MetricX_HumanRef| & 0.837 & 0.985 & 0.956 & 0.568 & 0.602 \\
\verb|COMET22_HumanRef_LLMRefine| & 0.811 & 0.97 & 0.988 & 0.405 & 0.578  \\
\verb|COMET22_HumanRef_HumanPEx2| & 0.811 & 0.97 & 0.988 & 0.401 & 0.577 \\
\verb|COMET22_HumanRef_HumanPE| & 0.811 & 0.97 & 0.988 & 0.406 & 0.577  \\
\verb|COMET22_HumanRef|     &  0.811 & 0.97 & 0.987 & 0.409 & 0.577  \\
\verb|BLEU_HumanRef_LLMRefine|  & 0.748 & 0.924 & 0.93 & 0.139 & 0.532 \\
\verb|BLEU_HumanRef_e2|  & 0.742 & 0.924 & 0.942 & 0.101 & 0.523  \\
\verb|BLEU_HumanRef|    & 0.741 & 0.909 & 0.938 & 0.133 & 0.518 \\
\verb|BLEU_HumanRef_e1|  & 0.738 & 0.894 & 0.935 & 0.135 & 0.521 \\
\bottomrule
\end{tabularx}
\caption{Meta evaluation results on English-German system-level and segment-level tasks from MetricX, COMET22 and BLEU with reference quality from various systems. The average correlation scores in the leftmost column takes an average of the results from the 4 main tasks. Rows are sorted by the overall average correlation scores.}
\label{tab:ende-mtme}
\end{table*}

==> tables/table_ende_post_edit_category.tex <==
\begin{table*}
\centering
\begin{adjustbox}{width=0.95\textwidth}

\begin{tabular}{l|l|c|l|c|l|c}
\hline
\multicolumn{1}{C{0.1cm}|}{} & \multicolumn{2}{c|}{\textbf{Accuracy}} & \multicolumn{2}{c|}{\textbf{Fluency}} & \multicolumn{2}{c}{\textbf{Style}} \\
\hline
\multirow{5}{*}{HumanPE \& LLMRefine} & Mistranslation & 70 & Grammar & 45 & Unnatural or awkward & 82 \\
& \multicolumn{1}{l|}{Creative Reinterpret} & 16 & Punctuation & 34 & Bad sentence structure & 4 \\
& \multicolumn{1}{l|}{Src lang fragment} & 10 & Text-Breaking & 15 & & \\
& Omission & 9 & Spelling & 11 & & \\
& Addition & 1 & Inconsistency & 8 & & \\
\cline{2-7}
& \multicolumn{2}{c|}{106} & \multicolumn{2}{c|}{121} & \multicolumn{2}{c}{86} \\
\hline
\multirow{5}{*}{HumanPE Only} & Mistranslation & 19 & Grammar & 14 & Unnatural or awkward & 27 \\
& \multicolumn{1}{l|}{Creative Reinterpret} & 17 & Punctuation & 8 & & \\
& \multicolumn{1}{l|}{Src lang fragment} & 4 & Text-Breaking & 3 & & \\
& Omission & 8 & Spelling & 2 & & \\
& Addition & 7 & Inconsistency & 1 & & \\
\cline{2-7}
& \multicolumn{2}{c|}{55} & \multicolumn{2}{c|}{29} & \multicolumn{2}{c}{27} \\
\hline
\multirow{5}{*}{LLMRefine Only} & Mistranslation & 57 & Grammar & 13 & \bf Unnatural or awkward & \bf 82 \\
& \multicolumn{1}{l|}{Creative Reinterpret} & 19 & Punctuation & 11 & Bad sentence structure & 5 \\
& \multicolumn{1}{l|}{Src lang fragment} & 7 & Text-Breaking & 3 & & \\
& Omission & 2 & Spelling & 7 & & \\
& Addition & 5 & Inconsistency & 3 & & \\
\cline{2-7}
& \multicolumn{2}{c|}{90} & \multicolumn{2}{c|}{42} & \multicolumn{2}{c}{87} \\
\hline
\end{tabular}
\end{adjustbox}
\caption{Error category statistics of different agreement sections of English-German translations}
\label{tab:ende-post-edit-category}
\end{table*}


==> tables/table_ende_post_edit_winloss.tex <==
% \begin{table}[htbp]
%     \centering
%     \begin{adjustbox}{width=0.98\columnwidth}
%     \begin{tabular}{lcccccccc}
%     \toprule
%     & \multicolumn{4}{c}{\textbf{HumanPE}} & \multicolumn{4}{c}{\textbf{LLMRefine}} \\
%     \cmidrule(lr){2-5} \cmidrule(lr){6-9}
%     \textbf{System} & \textbf{Win/Loss} & \textbf{Baseline} & \textbf{Win} & \textbf{Loss} & \textbf{Win/Loss} & \textbf{Baseline} & \textbf{Win} & \textbf{Loss} \\
%     \midrule
%     HumanRef & 2.13 & 1.01 & -3.4 & +4.1 & 2.16 & 1.61 & -4.9 & +3.0 \\
%     BestWMT & 1.88 & 1.33 & -3.5 & +4.8 & 1.19 & 1.08 & -3.5 & +4.5 \\
%     MidWMT & 3.58 & 0.80 & -6.5 & +5.4 & 3.76 & 1.22 & -6.6 & +4.6 \\
%     \bottomrule
%     \end{tabular}
%     \end{adjustbox}
%     \caption{Post-edit Win/Loss Ratio and average MQM Score Changes.}
%     \label{tab:ende-post-edit-winloss}
% \end{table}

\begin{table}[!htp]
\centering
\begin{adjustbox}{width=0.98\columnwidth}
\begin{tabular}{@{}lccc@{}}
\toprule
\textbf{Initial Trans.} & \textbf{Metric} & \textbf{HumanPE} & \textbf{LLMRefine} \\
\midrule
\multirow{3}{*}{HumanRef} 
 & Win/Loss & 2.13 & 2.16 \\
 \cline{2-4}
%  & Baseline & 1.01 & 1.61 \\
 & Win & -3.4 & -4.9 \\
 & Loss & +4.1 & +3.0 \\
\midrule
\multirow{3}{*}{BestWMT} 
 & Win/Loss & 1.88 & 1.19 \\
 \cline{2-4}

%  & Baseline & 1.33 & 1.08 \\
 & Win & -3.5 & -3.5 \\
 & Loss & +4.8 & +4.5 \\
\midrule
\multirow{3}{*}{MidWMT} 
 & Win/Loss & 3.58 & 3.76 \\
 \cline{2-4}

%  & Baseline & 0.80 & 1.22 \\
 & Win & -6.5 & -6.6 \\
 & Loss & +5.4 & +4.6 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Post-edit Win/Loss Ratio and average MQM Score Changes. Win/Loss represents the ratio of improved segments to degraded segments. Win and Loss values are average MQM score changes in improved/degraded segments; negative values indicate quality improvement (lower MQM score is better). }
\label{tab:ende-post-edit-winloss}
\end{table}

% Baseline reflects MQM score variance on unchanged translations.

==> tables/table_ende_qe_quality.tex <==
\begin{table}
\centering
\begin{adjustbox}{width=0.95\textwidth}
\begin{tabular}{lccccc}
\hline
\textbf{Reference} & \textbf{All}  & \textbf{news} & \textbf{mastodon} & \textbf{speech} & \textbf{user review}\\
\hline
\verb|new_ref_LLMRefine| & 1.24 & 0.88 & 1.03 & 2.13 & 1.17     \\
\verb|new_ref_e2| & 1.34 & 0.99	& 1.13  &	2.25 & 1.21 \\
\verb|new_ref_e1|   &  1.44	 & 0.87 &	1.18  &	2.46 &	1.65    \\
\verb|best_mt_LLMRefine|  & 1.46 & 	1.13 &	1.13 &	2.78 &	1.1    \\
\verb|best_wmt_postedit|  & 1.48 & 	0.91   &	1.24 &	2.86 &	1.22   \\
\verb|mid_wmt_postedit|  & 1.53	& 1.04	& 1.22	& 2.81	& 1.42   \\
\verb|new_ref|          & 1.54	 &1.1 & 1.23 & 2.5 & 1.73     \\
\verb|orig_ref|        &	1.56	& 1.18	& 1.35	& 2.71  &	1.18    \\
\verb|mid_mt_LLMRefine| & 1.64	& 1.47	& 1.14	& 2.66	& 1.78  \\
\verb|best_wmt_mt|    &   1.75	& 1.43	 &1.39 &	3.05 &	1.46     \\
\verb|mid_wmt_mt|   &     2.74	& 2.53 &	2.11 &	3.54	& 3.52     \\
\end{tabular}
\end{adjustbox}
% TODO: Better description of the table
\caption{English-German Data Collection Quality measured by Metric-X QE scores.}
\label{tab:zhen_qe_quality}
\end{table}

==> tables/table_finetune.tex <==
\begin{table}[!htb]
    \centering
    \begin{adjustbox}{width=0.98\columnwidth}
    \begin{tabular}{l|cc|c}
        \toprule
        \bf System & \bf MetricX & \bf COMET22 & \bf MQM Score \\
        \midrule
        \textsc{OrigHumanRef} & 2.96 & 0.829 & 5.63 (Tier-5) \\
        \textsc{HumanRef} & 2.83  & 0.829 & 2.05 (Tier-2) \\
        \textsc{HumanRef+HumanPE} & 2.80  & 0.829 & 1.91 (Tier-1) \\
        \textsc{HumanRef+HumanPEx2} & 2.73  & \bf 0.831 & \bf 1.82 (Tier-1) \\
        \textsc{HumanRef+LLMRefine} & \bf 2.65  & \bf 0.831 & \bf 1.82 (Tier-1) \\
        \midrule
        \textsc{BestWMT} & 3.08  & 0.830 & 2.22 (Tier-2) \\
        \textsc{BestWMT+HumanPE} & \bf2.88  & \bf 0.832 & \bf 1.87 (Tier-1) \\
        \textsc{BestWMT+LLMRefine} & 3.06  & 0.829 &  1.94 (Tier-1) \\
        \midrule
        \textsc{MidWMT} & 3.37  & 0.826 & 3.98 (Tier-4) \\
        \textsc{MidWMT+HumanPE} & \bf 2.88  & \bf 0.832 & \bf 2.23 (Tier-2) \\
        \textsc{MidWMT+LLMRefine} & 3.13 & 0.828 & 2.45 (Tier-3) \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Evaluation results of the Gemini-Nano models fine-tuned by datasets with varying MQMscores. Model has higher quality with higher COMET22 and lower MetricX scores.}
    \label{tab:zhen_finetune_comparison}
\end{table}

==> tables/table_mt_bias.tex <==
\begin{table}[!htp]
    \centering
    \begin{adjustbox}{width=0.98\columnwidth}
    \begin{tabular}{C{2cm}|C{2.2cm}|C{2cm}C{2cm}}
    \toprule
    \textbf{System} & \textbf{HumanRef\protect\newline+HumanPEx2}  & \textbf{BestWMT\protect\newline+HumanPE} & \textbf{MidWMT\protect\newline+HumanPE}\\
    \midrule
    Gemini & 1.35 & 1.26 (-0.09) & 1.23 (-0.12)\\
    BestWMT & 1.64 & \bf 1.12 (-0.52) & 1.41 (-0.23) \\
    ONLINE-W & 1.69 & 1.58 (-0.11) & 1.46 (-0.23) \\
    ONLINE-A & 2.24 & 2.15 (-0.09) & 1.96 (-0.27)\\
    MidWMT & 2.64 & 2.53 (-0.11) & \bf 2.24 (-0.39)\\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{MetircX Scores for English-German MT systems under reference translations with machine-based initial translations. Comparison to HumanRef+HumanPEx2 baseline reveals the bias from initial translations. The largest bias is highlighted.}
    \label{table:ende-bias-init-translation}
\end{table}

\begin{table}[!htp]
    \centering
    \begin{adjustbox}{width=0.98\columnwidth}
    \begin{tabular}{C{2cm}|C{3cm}|C{3cm}}
    \toprule
    \textbf{System} & \textbf{HumanRef\protect\newline+HumanPEx2}  & \textbf{HumanRef\protect\newline+LLMRefine}\\
    \midrule
    Gemini & 1.35 & 1.32 (-0.03)\\
    BestWMT & 1.64 & 1.67 (0.03) \\
    ONLINE-W & 1.69 & 1.75 (0.06)\\
    ONLINE-A & 2.24 & 2.34 (0.1)\\
    MidWMT & 2.64 & 2.71 (0.07)\\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{MetircX Scores for English-German MT systems under reference translations with machine-based post-edit approaches. Comparison to HumanRef+HumanPEx2 baseline reveals the bias from post-edit approaches. No significant large bias are presented.}
    \label{table:ende-bias-post-edit}
\end{table}

\begin{table}[!htp]
    \centering
    \begin{adjustbox}{width=0.98\columnwidth}
    \begin{tabular}{C{2cm}|C{2.2cm}|C{2cm}C{2cm}}
    \toprule
    \textbf{System} & \textbf{HumanRef\protect\newline+HumanPEx2}  & \textbf{BestWMT\protect\newline+LLMRefine} & \textbf{MidWMT\protect\newline+LLMRefine}\\
    \midrule
    Gemini & 1.35 & 1.28 (-0.07) & 1.19 (-0.16) \\
    BestWMT & 1.64 & \bf 1.12 (-0.51) & 1.49 (-0.15) \\
    ONLINE-W & 1.69 & 1.71 (0.02) & 1.62 (-0.07) \\
    ONLINE-A & 2.24 & 2.21 (-0.03) & 2.05 (-0.19)\\
    MidWMT & 2.64 & 2.65 (0.01) & \bf 2.16 (-0.48)\\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{MetircX Scores for English-German MT systems under reference translations with machine-based initial translations and post-edit approaches. Comparison to HumanRef+HumanPEx2 baseline reveals the combined bias from both stages . The largest bias is highlighted.}
    \label{table:ende-bias-combined}
\end{table}

==> tables/table_mtme.tex <==
\begin{table*}[!htp]
\centering
\footnotesize
\begin{tabularx}{\textwidth}{lrr|rrr|rrr}
\toprule
\multicolumn{1}{l}{\bf lang} & & \multicolumn{1}{c}{\bf en-de,zh-en} & \multicolumn{1}{c}{\bf en-de} & \multicolumn{1}{c}{\bf en-de} & \multicolumn{1}{c}{\bf en-de} & \multicolumn{1}{c}{\bf zh-en} & \multicolumn{1}{c}{\bf zh-en} & \multicolumn{1}{c}{\bf zh-en}\\
\multicolumn{1}{l}{\bf level} & & \multicolumn{1}{c}{\bf sys} & \multicolumn{1}{c}{\bf sys} & \multicolumn{1}{c}{\bf seg} & \multicolumn{1}{c}{\bf seg} & \multicolumn{1}{c}{\bf sys} & \multicolumn{1}{c}{\bf seg} & \multicolumn{1}{c}{\bf seg} \\
\multicolumn{1}{l}{\bf corr{\_}fn} & & \multicolumn{1}{c}{\bf accuracy} & \multicolumn{1}{c}{\bf pearson} & \multicolumn{1}{c}{\bf pearson} & \multicolumn{1}{c}{\bf acc-t} & \multicolumn{1}{c}{\bf pearson} & \multicolumn{1}{c}{\bf pearson} & \multicolumn{1}{c}{\bf acc-t} \\
\multicolumn{1}{l}{\bf Metric} &\multicolumn{1}{c}{\bf avg-corr} &\multicolumn{1}{c}{\bf task1} &\multicolumn{1}{c}{\bf task2} &\multicolumn{1}{c}{\bf task3} &\multicolumn{1}{c}{\bf task4} &\multicolumn{1}{c}{\bf task5} &\multicolumn{1}{c}{\bf task6} &\multicolumn{1}{c}{\bf task7}\\
\midrule
% \verb|MetricX_BestWMT_HumanPE| & 0.818 & 0.925 & 0.956 & 0.571 & 0.612 & 0.890 & 0.664 & 0.540 \\
\verb|MetricX_HumanRef_HuamnPEx2|  & 0.817 & 0.925 & 0.956 & 0.569 & 0.604 & 0.897 & 0.669 & 0.535 \\
\verb|MetricX_HumanRef_LLMRefine| & 0.816 & 0.925 & 0.957 & 0.567 & 0.602 & 0.900 & 0.667 & 0.533 \\
\verb|MetricX_HumanRef_HumanPE|  & 0.815 & 0.918 & 0.957 & 0.567 & 0.603 & 0.894 & 0.671 & 0.534  \\
\verb|MetricX_HumanRef| & 0.814 &  0.918  & 0.957   & 0.566   & 0.602  & 0.890   & 0.673   & 0.535       \\
\verb|COMET22_HumanRef_LLMRefine| & 0.805      & 0.959   & 0.991  & 0.403  & 0.577   & 0.978  & 0.462  & 0.526  \\
\verb|COMET22_HumanRef_HumanPEx2| & 0.803      & 0.952   & 0.991  & 0.398  & 0.576  & 0.980  & 0.462  & 0.527  \\
\verb|COMET22_HumanRef_HumanPE| & 0.802      & 0.952   & 0.991  & 0.404  & 0.576   & 0.980  & 0.452  & 0.526   \\
\verb|COMET22_HumanRef|     & 0.799      & 0.938   & 0.991 & 0.407  & 0.576   & 0.979  & 0.448  & 0.524  \\
\verb|BLEU_HumanRef|    & 0.744      & 0.932  & 0.934  & 0.134  & 0.520  & 0.913  & 0.201  & 0.480 \\
\verb|BLEU_HumanRef_LLMRefine|  & 0.743     & 0.911  & 0.934  & 0.141  & 0.533  & 0.932  & 0.207  & 0.482 \\
\verb|BLEU_HumanRef_e1|  & 0.742    & 0.918  & 0.935  & 0.136  & 0.523  & 0.922  & 0.204  & 0.482    \\
\verb|BLEU_HumanRef_e2|  & 0.740     & 0.911  & 0.929  & 0.102 & 0.523   & 0.947  & 0.213  & 0.483  \\
\bottomrule
\end{tabularx}
\caption{Meta evaluation results on English-German system-level and segment-level tasks from MetricX, COMET22 and BLEU with reference quality from various systems. The average correlation scores in the leftmost column takes a average of the results from the 4 main tasks, including system-level and segment-level tasks. Rows are sorted by the overall average correlation scores.}
\label{tab:mtme}
\end{table*}

==> tables/table_zhen_mqm_domains.tex <==
\begin{table}[!htb]
    \centering
    \begin{adjustbox}{width=0.98\columnwidth}
    \begin{tabular}{lccc}
        \toprule
        \textbf{Reference} & \textbf{News} & \textbf{User Review} & \textbf{Manual}\\
        \midrule
        \textsc{HumanRef} & 2.57 & 1.75 & 2.03\\
        \textsc{HumanRef+HumanPE} & 2.45 & 1.61 & 1.86 \\
        \textsc{HumanRef+HumanPEx2} & 2.32 & 1.52 & 1.92\\
        \textsc{HumanRef+LLMRefine} & 2.04 & 1.64 & 2.13 \\
        \textsc{BestWMT} & 2.24 & 2.35 & 1.45\\
        \textsc{BestWMT+HumanPE} & 2.09 & 1.85 & 1.33 \\
        \textsc{BestWMT+LLMRefine} & 2.10 & 1.96 & 1.28\\
        \textsc{MidWMT} & 3.71 & 4.45 & 2.19 \\
        \textsc{MidWMT+HumanPE} & 2.29 & 2.28 & 1.74 \\
        \textsc{MidWMT+LLMRefine} & 2.62 & 2.49 & 1.67\\
        \textsc{OrigHumanRef} & 5.49 & 5.20 & 8.43\\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Chinese-English MQM human evaluations for generalMT2023 with different systems under different domains.}
    \label{tab:zhen_mqm_domains}
\end{table}

==> tables/table_zhen_mtme.tex <==
\begin{table*}[!htp]
\centering
\footnotesize
\begin{tabularx}{0.75\textwidth}{lr|rrrr}
\toprule
\multicolumn{1}{l}{\bf Metric} & \multicolumn{1}{c}{\bf avg-corr} & \multicolumn{1}{c}{\bf en-de} & \multicolumn{1}{c}{\bf en-de} & \multicolumn{1}{c}{\bf en-de} & \multicolumn{1}{c}{\bf en-de}\\
\multicolumn{1}{l}{\bf level} & & \multicolumn{1}{c}{\bf sys} & \multicolumn{1}{c}{\bf sys} & \multicolumn{1}{c}{\bf seg} & \multicolumn{1}{c}{\bf seg} \\
\multicolumn{1}{l}{\bf corr{\_}fn} & & \multicolumn{1}{c}{\bf accuracy} & \multicolumn{1}{c}{\bf pearson} & \multicolumn{1}{c}{\bf pearson} & \multicolumn{1}{c}{\bf acc-t} \\
\multicolumn{1}{l}{\bf task} & & \multicolumn{1}{c}{\bf task1} & \multicolumn{1}{c}{\bf task2} & \multicolumn{1}{c}{\bf task3} & \multicolumn{1}{c}{\bf task4}\\
\midrule
\verb|MetricX_HumanRef_HuamnPEx2|  & 0.805 & 0.895 & 0.901 & 0.668 & 0.541 \\
\verb|MetricX_HumanRef_LLMRefine| & 0.805 & 0.895 & 0.903 & 0.666 & 0.539 \\
\verb|MetricX_HumanRef_HumanPE|  & 0.805 & 0.895 & 0.897 & 0.67 & 0.54  \\
\verb|MetricX_HumanRef| & 0.805 & 0.895 & 0.896 & 0.672 & 0.54 \\
\verb|COMET22_HumanRef_HumanPE| & 0.79 & 0.924 & 0.96 & 0.453 & 0.53   \\
\verb|COMET22_HumanRef|     & 0.789 & 0.924 & 0.96 & 0.449 & 0.528  \\
\verb|COMET22_HumanRef_HumanPEx2| & 0.787 & 0.905 & 0.959 & 0.463 & 0.531  \\
\verb|COMET22_HumanRef_LLMRefine| & 0.786 & 0.905 & 0.957 & 0.462 & 0.53  \\
\verb|BLEU_HumanRef_e2|  & 0.74 & 0.905 & 0.941 & 0.208 & 0.482  \\
\verb|BLEU_HumanRef_LLMRefine|  & 0.728 & 0.867 & 0.928 & 0.203 & 0.482 \\
\verb|BLEU_HumanRef_e1|  & 0.722 & 0.857 & 0.903 & 0.2 & 0.48 \\
\verb|BLEU_HumanRef|    & 0.72 & 0.857 & 0.889 & 0.196 & 0.479 \\
\bottomrule
\end{tabularx}
\caption{Meta evaluation results on Chinese-English system-level and segment-level tasks from MetricX, COMET22 and BLEU with reference quality from various systems. The average correlation scores in the leftmost column takes an average of the results from the 4 main tasks. Rows are sorted by the overall average correlation scores.}
\label{tab:zhen-mtme}
\end{table*}
